Flow and Transport in Three-Dimensional Discrete Fracture Matrix Models using Mimetic Finite Difference on a Conforming Multi-Dimensional Mesh

We present a comprehensive workflow to simulate single-phase flow and transport in fractured porous media using the discrete fracture matrix approach. The workflow has three primary parts: (1) a method for conforming mesh generation of and around a three-dimensional fracture network, (2) the discretization of the governing equations using a second-order mimetic finite difference method, and (3) implementation of numerical methods for high-performance computing environments. A method to create a conforming Delaunay tetrahedralization of the volume surrounding the fracture network, where the triangular cells of the fracture mesh are faces in the volume mesh, that addresses pathological cases which commonly arise and degrade mesh quality is also provided. Our open-source subsurface simulator uses a hierarchy of process kernels (one kernel per physical process) that allows for both strong and weak coupling of the fracture and matrix domains. We provide verification tests based on analytic solutions for flow and transport, as well as numerical convergence. We also provide multiple expositions of the method in complex fracture networks. In the first example, we demonstrate that the method is robust by considering two scenarios where the fracture network acts as a barrier to flow, as the primary pathway, or offers the same resistance as the surrounding matrix. In the second test, flow and transport through a three-dimensional stochastically generated network containing 257 fractures is presented.

==> sections/graph_backbone.tex <==
% backbone text adapted from Osthus et al 2010

\jeffrey{graph representations details : Revise}
The discrete structure of a DFN naturally lends itself to various graph representations~\cite{andresen2013topology,hope2015topological,huseby1997geometry,hyman2019linking,karra2018modeling}.
The mathematical construct of a graph $G(\bV,\bE)$ is a set of vertices $\bV$, a set of edges $\bE$, and a rule that assigns which edges connect vertices. 
Similarly, the topology of a DFN can be described using a tuple $(\bF,\bI)$ where $\bF$ is the set of all fractures in the network and $\bI$ is the set of intersections between fractures~\cite{hyman2018identifying}. 
Formally, let $\bF = \{f_i \}$ for $i=1,\ldots, n$ denote a fracture network composed of $n$ fractures and $\bI = \{(f_i, f_j)\}$  be a set of pairs associated with intersections between fractures; if $f_i  \cap f_j \ne \emptyset$ then $(f_i, f_j) \in \bI$.
The number of intersections $m=|\bI|$ depends on the particular shape, orientation, and geometry of the set of fractures in the network.

We use the graph representation of a DFN presented by al.~\cite{hyman2017predictions}, where vertices in the graph correspond to fractures in the network ($\bF$) and edges indicated that two fractures intersect ($\bI$).
Let $\phi$ define an isomorphic mapping that transforms $(\bF,\bI)$ into a graph $G \equiv G(\bV,\bE)$ where $\bV$ is a set of  of $n=|\bV|$ vertices and $\bE$ is a set of $m=|\bE|$ edges.
For every $f_i \in \bF $, there is a unique vertex $v_i \in \bV$, 
\begin{linenomath*}
\begin{equation}\label{eq:phi1}
\phi : f_i \rightarrow v_i \,.
\end{equation}
\end{linenomath*}
If two fractures, $f_i$ and $f_j$, intersect $ (f_i,f_j) \in \bI$, then there is an edge in $\bE$ connecting the corresponding vertices, 
\begin{linenomath*}
\begin{equation}\label{eq:phi2}
\phi : f_i \cap f_j \ne \emptyset \rightarrow e_{ij} = (v_i,v_j)\,,
\end{equation}
\end{linenomath*}
where $(v_i,v_j)\in \bE$ denotes an edge between vertices $v_i$ and $v_j$.
We also include source $s$ and target $t$ vertices into $\bV$ to incorporate flow direction.
Every fracture that intersects the inlet plane $\vx_0$ is connected to the source vertex, 
\begin{linenomath*}
\begin{equation}
\phi : f_i \cap \vx_0 \ne \emptyset \rightarrow e_{si} = (s,v_i)\,,
\end{equation}
\end{linenomath*}
and every fracture that intersects the outlet plane $\vx_L$ is connected to the target vertex $t$,
\begin{linenomath*}
\begin{equation}
\phi : f_i \cap \vx_L \ne \emptyset \rightarrow e_{it} = (v_i,t)\,.
\end{equation}
\end{linenomath*}


\begin{figure*}[htb!] \centerline{
 \begin{tabular}{cc}
\includegraphics[width=0.45\textwidth]{figures/graph.png} 
 \end{tabular}}
\caption{\label{fig:backbone_graph} }
\end{figure*}

\jeffrey{Note we use the 2-core and explain why}

\jeffrey{Image of DFN / graph / DFN - backbone /Backbone graph}



\subsubsection{Upscaling}

The equivalent porosity of a matrix cell intersected by at least one secondary fracture is given by
	\begin{equation}
		\phi=\frac{V_t}{V_c}
	\end{equation}
where $V_t$ is the total volume of $N$ intersecting fractures in the cell and $V_c$ is the volume of the cell.  $V_t$ is given by the estimation
	\begin{equation}
		V_t=\sum^N_{f=1}V_{f}=\sum^N_{f=1}A_{f}b_f
	\end{equation}
with fracture areas $A_{f}$ and apertures $b_f$.  

The equivalent fracture permeability tensor can be defined at each cell in the matrix mesh by 
	\begin{equation}
		\bm{K}_f=\frac{1}{12}\sum^N_{f=1}\phi_{f}b_{f}^2\bm{\Omega}_f
	\end{equation}
where $\phi_{f}$ is the porosity of fracture $f$ at the cell and $\bm{\Omega}_f$ is a coordinate transformation tensor given by
	\begin{equation}
		\bm{\Omega}_f=
			\begin{bmatrix}
				(n_2)^2 +(n_3)^2 & -n_1n_2 & -n_3n_1\\
				-n_1n_2 & (n_3)^2+(n_1)^2 & -n_2n_3\\
				-n_3n_1 & -n_2n_3 & (n_1)^2+(n_2)^2
			\end{bmatrix}
	\end{equation}
where $n_1,n_2,n_3$ are the components of the normal vector of fracture $f$.

In cases where the matrix has a non-neglible permeability, the permeability value is assumed to be a weighted arithmetic average of the fracture and matrix permeability values. In addition, for fractures that are not parallel to one of the coordinate axes, the permeability needs to be corrected to account for the artificially long flow paths caused by the discretized mesh (see Sweeney et al. \cite{sweeney2019upscaled}).


